Unleashing the Power of LLM to Infer State Machine from the Protocol Implementation

State machines are essential for enhancing protocol analysis to identify vulnerabilities. However, inferring state machines from network protocol implementations is challenging due to complex code syntax and semantics. Traditional dynamic analysis methods often miss critical state transitions due to limited coverage, while static analysis faces path explosion issues. To overcome these challenges, we introduce a novel state machine inference approach utilizing Large Language Models (LLMs), named ProtocolGPT. This method employs retrieval augmented generation technology to enhance a pre-trained model with specific knowledge from protocol implementations. Through effective prompt engineering, we accurately identify and infer state machines. To the best of our knowledge, our approach represents the first state machine inference that leverages the source code of protocol implementations. Our evaluation of six protocol implementations shows that our method achieves a precision of over 90%, outperforming the baselines by more than 30%. Furthermore, integrating our approach with protocol fuzzing improves coverage by more than 20% and uncovers two 0-day vulnerabilities compared to baseline methods.

==> table/table_demo.tex <==
\begin{table}[t]
\centering
\caption{The real-world programs used as benchmarks} \label{tab:exp-programs}

\resizebox{1.0\linewidth}{!}{
\begin{tabular}{ccc}
\toprule
\textbf{Program} & \textbf{Version} & \textbf{Bug Type} \\

\midrule

guetzli & git (9afd0bb)  & Assertion Fail \\

\rowcolor[HTML]{EFEFEF} 
harfbuzz & git (f73a87d) & Assertion Fail \\
json & git (b04543e) & Assertion Fail \\

\rowcolor[HTML]{EFEFEF} 
lcms & git (f9d75cc)  & Heap Buffer Overflow \\
libarchive & git (51d7afd) & Heap Buffer Overflow \\

\rowcolor[HTML]{EFEFEF} 
libpng &  1.2.56 & Out Of Memory \\
libxml & v2.9.2 & Heap Buffer Overflow \\

\rowcolor[HTML]{EFEFEF}
openssl & 1.0.1f & Heap Buffer Overflow \\
pcre2 & 10.00 & Heap Use after Free \\

\rowcolor[HTML]{EFEFEF}
re2 & git (499ef7e) & Heap Buffer Overflow \\
vorbis & git (c1c2831) & Heap Buffer Overflow \\

\rowcolor[HTML]{EFEFEF}
woff2 & git (9476664) & Heap Buffer Overflow \\
\bottomrule
\end{tabular}
}
\end{table}

==> tex/Acknowledfments.tex <==
\begin{acks}
To Robert, for the bagels and explaining CMYK and color spaces.
\end{acks}

==> tex/RelatedWork.tex <==
\section{Related work}

\header{Natural Language Processing}
Pacheco et al. advanced a novel methodology for inferring protocol state machines, anchored in NLP and adopting a data-driven paradigm~\cite{pacheco2022automated}. This method involves the training of deep learning models on a comprehensive corpus of natural language data, encompassing technical documentation and protocol specification documents. Subsequently, leveraging labeled data, this approach facilitates the derivation of relationships between variables within the protocol specifications via the model, culminating in the articulation of a finite state machine representative of the protocol.

% \vspace{3pt}
\header{Dynamic Analysis}
Kleber et al. unveiled a novel strategy for the categorization of message types within binary protocols~\cite{kleber2020message}. This strategy relies on a similarity metric using continuous value ranges to compare feature vectors based on message fields instead of discrete byte values, thereby facilitating an enhanced discernment of message format patterns. Further contributing to the field, Ye et al. advanced a probabilistic approach to the reversal of network protocols~\cite{ye2021netplier}. By constructing a joint distribution between these random variables and the observed values within messages, probabilistic reasoning is employed to ascertain potential keywords. Gopinath et al. introduced a comprehensive algorithm designed to deduce the syntax of inputs from programs, distinguishing itself by eschewing conventional data flow analysis methodologies~\cite{gopinath2020mining}. Uniquely, this methodology obviates the necessity for heuristic strategies traditionally employed to discern parsing patterns, rendering it universally applicable across all recursive parsers that operate on the basis of program stacks.

% \vspace{3pt}
\header{Static Analysis}
Shi et al. pioneered the development of a protocol state machine inference methodology predicated on static analysis~\cite{shi2023extracting}. This innovative approach employs static analysis to examine protocol formats derived from parsers within the protocol implementations. The extraction of state machines is achieved by interpreting each iteration of a loop as a distinct state, with the interdependencies among loop iterations being regarded as transitions between states.
